Expressing advanced user preferences in component installation

State of the art component-based software collections - such as FOSS distributions - are made of up to dozens of thousands components, with complex inter-dependencies and conflicts. Given a particular installation of such a system, each request to alter the set of installed components has potentially (too) many satisfying answers. We present an architecture that allows to express advanced user preferences about package selection in FOSS distributions. The architecture is composed by a distribution-independent format for describing available and installed packages called CUDF (Common Upgradeability Description Format), and a foundational language called MooML to specify optimization criteria. We present the syntax and semantics of CUDF and MooML, and discuss the partial evaluation mechanism of MooML which allows to gain efficiency in package dependency solvers.

==> upgrade.tex <==
\section{Packages and upgrades}
\label{sec:upgrade}

\emph{Packages} are abstractions defining the granularity at which
users can act (add, remove, upgrade, etc.) on available software. A
\emph{distribution} is a collection of packages maintained (hopefully)
coherently. The subset of a distribution corresponding to the actual
packages installed on a machine is called \emph{package status} and is
meant to be altered using the \emph{package manager} offered by a
given distribution.  An \emph{upgrade scenario} is the situation in
which a user---typically acting with system administrator
rights---submit a \emph{user request} to a given package manager, with
the intention to alter the current packages status. Several entities
and problems are involved in, and should be grasped by a complete
description of, an upgrade
scenario~\cite{hotswup:package-upgrades}. The main entities are
packages and the most relevant problem for the present paper is
upgrade planning; both are briefly described below.

Abstracting over format-specific details, a \emph{package} is a bundle
of 3 main parts:
\[\mathit{Package} \quad \left\{ \quad
\begin{tabular}{|ll|}
  \hline
  1. & Set of \emph{files} \\
  ~ 1.1. & ~ ~ \fbox{\emph{Configuration files}} \\[1ex]
  \hline\hline
  2. &  Set of valued \emph{meta-information} \\
  ~ 2.1. & ~ ~ \fbox{\emph{Inter-package relationships}} \\[1ex]
  \hline\hline
  3. &  Executable \emph{configuration scripts} \\
  \hline
\end{tabular} \right.\]
The set of files (1) is common in all software packaging solutions, it
is the filesystem encoding of what the package is delivering:
executable binaries, data, documentation, etc. Such set includes
configuration files (1.1), that affect the runtime behavior of the
package and are meant to be locally customized.  Package
meta-information (2) contains information varying from distribution to
distribution. A common core provides: a unique identifier, a (totally
ordered) software version, maintainer and package description, and
most notably \emph{inter-package relationships} (2.1). The
relationship kinds vary with the installer, but there exists a de
facto common subset including: dependencies (the need of other
packages to work properly), conflicts (the inability of being
co-installed with other packages), feature provisions (the ability to
declare named features as provided by a given package, so that other
packages can depend on them), and restricted boolean combinations of
them~\cite{edos-package-management}. Finally, packages come with a set
of executable configuration (or \emph{maintainer}) scripts (3). Their
purpose is to let package maintainers attach actions to hooks executed
by the installer; actions are used to finalize package configuration
during deployment.

\begin{table}[t]
 \begin{tabular}{l}
  %\textbf{Upgrade phase} & \textbf{Sample log}\\\hline
  \begin{minipage}[c]{\logwidth}
   \begin{Verbatim}[commandchars=\\\{\},fontsize=\logsize]
# apt-get install aterm\hfill\emph{1. user request}
   \end{Verbatim}
  \end{minipage}
  \\\hline
  \begin{minipage}[c]{\logwidth}
   \begin{Verbatim}[commandchars=\\\{\},fontsize=\logsize]
Reading package lists... Done\hfill\emph{2. dep.resolution}
Building dependency tree... Done
The following extra packages will be installed:
  libafterimage0
0 upgraded, 2 newly installed, 0 to remove and
  1786 not upgraded.
Need to get 386kB of archives.
807kB of additional disk space will be used.
   \end{Verbatim}
  \end{minipage}
  \\\hline
  \begin{minipage}[c]{\logwidth}
   \begin{Verbatim}[commandchars=\\\{\},fontsize=\logsize]
Get: 1 http://ftp.debian.org libafterimage0 2.2.8-2
Get: 2 http://ftp.debian.org aterm 1.0.1-4
Fetched 386kB in 0s (410kB/s)\hfill\emph{3. package retrieval}
   \end{Verbatim}
  \end{minipage}
  \\\hline
  \begin{minipage}[c]{\logwidth}
   \begin{Verbatim}[commandchars=\\\{\},fontsize=\logsize]
    \hfill\emph{5a. (pre-)configuration}
   \end{Verbatim}
  \end{minipage}
  \\\hline
  \begin{minipage}[c]{\logwidth}
   \begin{Verbatim}[commandchars=\\\{\},fontsize=\logsize]
Selecting package libafterimage0.\hfill\emph{4. unpacking}
(Reading database ... 294774 files and dirs installed.)
Unpacking libafterimage0 (libafterimage0_2.2.8-2_i386.deb)
Selecting package aterm.
Unpacking aterm (aterm_1.0.1-4_i386.deb) ...
   \end{Verbatim}
  \end{minipage}
  \\\hline
  \begin{minipage}[c]{\logwidth}
   \begin{Verbatim}[commandchars=\\\{\},fontsize=\logsize]
Setting up libafterimage0 (2.2.8-2) ...
Setting up aterm (1.0.1-4) ...\hfill\emph{5b. (post-)configuration}
   \end{Verbatim}
  \end{minipage}
 \end{tabular}

 \caption{The package upgrade process}
 \label{tab:upgrade-phases}
\end{table}

Table~\ref{tab:upgrade-phases} summarizes the different phases of the
\emph{upgrade process}, using as an example the popular
\texttt{apt-get} package manager (others follow a similar process).
Phase (1) is a user specification of how she wants the local package
status to be altered. The expressiveness of the language available to
formulate this \emph{user request} varies with the meta-installer: it
can be as simple as requesting the installation/removal of a single
package, or as complex as \texttt{apt-get} pinning that allows to
express preferences to discriminate among multiple versions of the
same package. Phase (2) performs dependency resolution: it checks
whether a package status satisfying all dependencies and implementing
the user request exists.\footnote{The problem is at least
  NP-complete~\cite{edos-package-management}.} If this is the case,
one is chosen in this phase and is called \emph{solution}. Deploying
the new status consists of package retrieval (3) and unpacking (4).
Intertwined with those phases there are several configuration phases
(5) where maintainer scripts get executed.

Various challenges related to the upgrade process still need to be
properly addressed. An example of a very practical challenge is the
need to provide transactional upgrades, which offer the possibility to
roll back in case an unexpected (and unpredictable in general) failure
is encountered during upgrade
deployment~\cite{hotswup:package-upgrades,mancoosi-wp1d1}. Other
challenges concern \emph{upgrade planning}. For instance, dependency
resolution can fail either because the user request is unsatisfiable
(e.g., user error or inconsistent distributions~\cite{edos2006ase}) or
because the package manager is unable to find a
solution. Completeness---the guarantee that a solution will be found
whenever one exists---is a desirable package manager
property~\cite{mancoosi-debconf8}, unfortunately missing in most
package managers, with too few claimed
exceptions~\cite{niemeyer-smart,tucker-opium}.

While SAT solving has been proven to be a suitable and complete
technique to solve dependencies~\cite{edos2006ase}, it is still
missing is wide adoption. \emph{Handling complex user preferences} is
a novel problem for software upgrade, and is the main concern of the
this paper. It boils down to let users specify which solution to
choose among all acceptable solutions. Example of preferences are
policies~\cite{niemeyer-smart,trezentos07}, like minimizing the
download size or prioritizing popular packages, and also more specific
requirements such as blacklisting packages maintained by an untrusted
maintainer.

The first required step to attack the problem is devising a way to
encode user preferences in a flexible way, still manageable by package
managers which will have to respect them while computing new package
statuses. A prerequisite of that, is a rigorous description of upgrade
scenarios, over which the meaning of user preferences will be
expressed.

